On The Communication Complexity of Linear Algebraic Problems in the Message Passing Model

We study the communication complexity of linear algebraic problems over finite fields in the multi-player message passing model, proving a number of tight lower bounds. Specifically, for a matrix which is distributed among a number of players, we consider the problem of determining its rank, of computing entries in its inverse, and of solving linear equations. We also consider related problems such as computing the generalized inner product of vectors held on different servers. We give a general framework for reducing these multi-player problems to their two-player counterparts, showing that the randomized $s$-player communication complexity of these problems is at least $s$ times the randomized two-player communication complexity. Provided the problem has a certain amount of algebraic symmetry, which we formally define, we can show the hardest input distribution is a symmetric distribution, and therefore apply a recent multi-player lower bound technique of Phillips et al. Further, we give new two-player lower bounds for a number of these problems. In particular, our optimal lower bound for the two-player version of the matrix rank problem resolves an open question of Sun and Wang. A common feature of our lower bounds is that they apply even to the special "threshold promise" versions of these problems, wherein the underlying quantity, e.g., rank, is promised to be one of just two values, one on each side of some critical threshold. These kinds of promise problems are commonplace in the literature on data streaming as sources of hardness for reductions giving space lower bounds.

==> conclusion.tex <==
\section{Conclusion}
\label{sec:con}

In this paper we proved several new lower bounds on the communication complexity of
natural problems occurring in linear algebra, via the the rank promise problem. 
The matrices we considered here are over $\mathbb{F}_p$. It is an interesting open question to consider these problems over $\mathbb Z$ with some bound on the magnitude of the coefficients. 

These linear algebra problems have also been studied in cryptographic settings, see, e.g., \cite{nw06}, where our result shows that their bounds are near-optimal even for insecure communication and even with the promise that the players hold disjoint subspaces or that their subspaces intersect in a $1$-dimensional space. Another application of our results is to property testing, for which the results \cite{sun2012randomized} we improve upon have recently found applications \cite{gwx13}.

%, where they mention that determining the randomized communication complexity of subspace intersection as an open problem 
%
% Many constructions in cryptography are based on algebraic problems over finite fields. In the communication complexity, we show that Alice and Bob have to transfer much information to compute these functions. One could find the relationship to cryptography and show the secret is safe unless revealing a lot of information.


==> predefs.tex <==
\bibliographystyle{splncs03}


\spnewtheorem{fact}[theorem]{Fact}{\bfseries}{\itshape}

\DeclareMathOperator{\pre}{pre}
\DeclareMathOperator{\cost}{cost}
\DeclareMathOperator{\rk}{rank}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\IC}{IC}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\PRIV}{PRIV} 
\DeclareMathOperator{\wt}{wt}

\newcommand{\pub}{\textrm{pub}}
\newcommand{\rankp}{{\rk}}
\newcommand{\size}{{\operatorname{size}}}
\newcommand{\detp}{{\operatorname{det}_p}}
\newcommand{\disc}{{\operatorname{disc}}}
\newcommand{\tr}{{\operatorname{tr}}}
\newcommand{\diag}{{\operatorname{diag}}}
\newcommand{\argmax}{{\operatorname{argmax}}}
\newcommand{\sign}{{\operatorname{sign}}}

\newcommand{\trans}{^\mathrm{T}}

\newcommand{\scdet}{\textsc{Det}}
\newcommand{\scsin}{\textsc{Singularity}}
\newcommand{\scrp}{\textsc{RankParity}}
\newcommand{\scrank}{\textsc{Rank}}
\newcommand{\scinv}{\textsc{Inverse}}
\newcommand{\scip}{\textsc{IP}}
\newcommand{\scsls}{\textsc{SolveLinearSystem}}

\newcommand{\D}{\ensuremath\mathcal{D}}
\newcommand{\G}{\ensuremath\mathcal{G}}
\newcommand{\F}{\ensuremath\mathbb{F}}


\allowdisplaybreaks

